FedCAT: Towards Accurate Federated Learning via Device Concatenation

As a promising distributed machine learning paradigm, Federated Learning (FL) enables all the involved devices to train a global model collaboratively without exposing their local data privacy. However, for non-IID scenarios, the classification accuracy of FL models decreases drastically due to the weight divergence caused by data heterogeneity. Although various FL variants have been studied to improve model accuracy, most of them still suffer from the problem of non-negligible communication and computation overhead. In this paper, we introduce a novel FL approach named Fed-Cat that can achieve high model accuracy based on our proposed device selection strategy and device concatenation-based local training method. Unlike conventional FL methods that aggregate local models trained on individual devices, FedCat periodically aggregates local models after their traversals through a series of logically concatenated devices, which can effectively alleviate the model weight divergence problem. Comprehensive experimental results on four well-known benchmarks show that our approach can significantly improve the model accuracy of state-of-the-art FL methods without causing extra communication overhead.

==> reference.tex <==
\begin{thebibliography}{plainnat}



\bibitem{communication}
B.~McMahan, E.~Moore, D.~Ramage, S.~Hampson, B.~Arcas,
  Communication-efficient learning of deep networks from decentralized
  data, in: Proc. of International Conference on
  Artificial Intelligence and Statistics (AISTATS), vol.~54, 2017, pp. 1273--1282.


               
               
\bibitem{largescale}
L.~Bottou, Large-scale machine learning with stochastic gradient descent,
  in: Proc. of International Conference on Computational Statistics (COMPSTAT), 2010, pp. 177--186.






\bibitem{hfl}
H.~Yang,
  H-FL: A hierarchical communication-efficient and privacy-protected
               architecture for federated learning, in: Proc. of International Joint Conference on Artificial
               Intelligence (IJCAI), 2021, pp. 479--485.
               
               
\bibitem{spars}
R.~Hu, Y.~Gong, Y.~Guo,
  Federated learning with sparsification-amplified privacy and adaptive
               optimization, in: Proc. of International Joint Conference on Artificial
               Intelligence (IJCAI), 2021, pp. 1463--1469.



\bibitem{practical}
L.~Sun, J.~Qian, X.~Chen,
  {LDP-FL:} Practical private aggregation in federated learning with
               local differential privacy, in: Proc. of International Joint Conference on Artificial
               Intelligence (IJCAI), 2021, pp. 1571--1578.



\bibitem{oneshot}
Q.~Li, B.~He, D.~Song,
Practical one-shot federated learning for cross-silo setting, in: Proc. of International Joint Conference on Artificial
               Intelligence (IJCAI), 2021, pp. 1484--1490.
               
               
               
               
\bibitem{fair}
Z.~Wang, X.~Fan, J.~Qi, C.~Wen, C.~Wang, R.~Yu,
Federated learning with fair averaging, in: Proc. of International Joint Conference on Artificial
               Intelligence (IJCAI), 2021, pp. 1615--1623.
               
               
               
\bibitem{mimics}
H.~Huang, F.~Shang, Y.~Liu, H.~Liu,
Behavior mimics distribution: combining individual and group behaviors
               for federated learning, in: Proc. of International Joint Conference on Artificial
               Intelligence (IJCAI), 2021, pp. 2556--2562.



\bibitem{advance}
P.~Kairouz et al., Advances and open problems in Federated Learning,
  Foundations and Trends in Machine Learning, vol.~14, no.~1--2, pp. 1--210, 2021.
  
  


\bibitem{convergence}
X.~Li, K.~Huang, W.~Yang, S.~Wang, Z.~Zhang, On the convergence of fedAvg on non-IID data, in: Proc. of International Conference on Learning Representations (ICLR), 2020, pp. 1--12.





\bibitem{scaffold}
S. Karimireddy, S. Kale, M. Mohri, S. Reddi, S. Stich, A. Suresh, {SCAFFOLD:} stochastic controlled averaging for on-device federated
  learning, arXiv:1910.06378, 2019, pp. 1--12.


\bibitem{noniid}
Y.~Zhao, M.~Li, L.~Lai, N.~Suda, D.~Civin, V.~Chandra, Federated Learning with Non-IID Data, arXiv:1806.00582, 2018, pp. 1--13.




\bibitem{multicenter}
M.~Xie, G.~Long, T.~Shen, T.~Zhou, X.~Wang, and J.~Jiang, Multi-center federated learning, arXiv:2108.08647, 2021, pp. 1--12.
  


\bibitem{hierarchical}
C.~Briggs, Z.~Fan, and P.~Andras, ``Federated learning with hierarchical
  clustering of local updates to improve training on non-iid data''. in \emph{Proc. of International Joint Conference on Neural Networks (IJCNN)}, 2020,
  pp. 1--9.
  


\bibitem{crosssilo}
Y. Huang, L. Chu, Z. Zhou, L. Wang, J. Liu, J. Pei, Y. Zhang,
  Personalized cross-silo federated learning on non-IID data, in: Proc. of Applications of Artificial Intelligence (AAAI), 2021, pp. 7865--7873.
  
  

\bibitem{ensembledist}
T. Lin, L. Kong, S. Stich, M. Jaggi, Ensemble distillation for robust model fusion in federated learning, in: Proc. of Annual Conference
               on Neural Information Processing Systems (NeurIPS), 2020, pp. 1--13.
               
               
               
\bibitem{feded}
D. Sui, Y. Chen, J. Zhao, Y. Jia, Y. Xie, W. Sun,
  FedED: Federated learning via ensemble distillation for medical relation
               extraction, in: Proc. of Conference on Empirical Methods in Natural
               Language Processing (EMNLP), 2020, pp. 2118--2128.
               
               
               
               
\bibitem{datafree}
Z.~Zhu, J.~Hong, J.~Zhou,
Data-free knowledge distillation for heterogeneous federated learning, in: Proc. of International Conference on Machine Learning (ICML), 2021, pp. 12878--12889.




\bibitem{curiosity}
Y.~Zheng, Y.~Liu, X.~Xie, Y.~Liu, L.~Ma, J.~Hao, Y.~Liu,
  Automatic web testing using curiosity-driven reinforcement learning, in: Proc. of International Conference on Software Engineering (ICSE), 2017, pp. 423--435.



\end{thebibliography}
